Connecting First and Second Order Recurrent Networks with Deterministic Finite Automata

We propose an approach that connects recurrent networks with different orders of hidden interaction with regular grammars of different levels of complexity. We argue that the correspondence between recurrent networks and formal computational models gives understanding to the analysis of the complicated behaviors of recurrent networks. We introduce an entropy value that categorizes all regular grammars into three classes with different levels of complexity, and show that several existing recurrent networks match grammars from either all or partial classes. As such, the differences between regular grammars reveal the different properties of these models. We also provide a unification of all investigated recurrent networks. Our evaluation shows that the unified recurrent network has improved performance in learning grammars, and demonstrates comparable performance on a real-world dataset with more complicated models.

==> base/backup.tex <==


On the theoretical front, understanding of RNNs is at best rudimentary. With the current techniques,
it is not tractable to analyze the highly non-linear state evolution in RNNs. Analysis of backpropagation
is also intractable due to non-convexity of the loss function, and in general, reaching the global optimum
is hard. Here, we take the first steps towards addressing these challenging issues. We design novel spectral
methods for training IO-RNN and BRNN models.

The reasons for making formal languages the
targets of learning are as valid today as they were
decades ago. First, the grammars generating the
formal languages are known. Therefore training
and test data can be generated as desired. Thus,
the scientist can run controlled experiments to see
whether particular generalizations are reliably acquired
under particular training regimens.

Importantly, the relative complexity of different
formal languages may provide additional insight.
If it is found that formal languages of one
type are more readily learned than formal languages
of another type in some set of experiments
then the difference between these classes may be
said to meaningfully capture some property unavailable
to the RNNs in the experiments. Subsequent
work may lead to proofs and theorems about
which properties of RNNs lead to the reliable inference
of formal languages from certain classes and which do not. It may also lead to new network
architectures which overcome identified hurdles.
